Safety, Trust, and Ethics Considerations for Human-AI Teaming in Aerospace Control

Designing a safe, trusted, and ethical AI may be practically impossible; however, designing AI with safe, trusted, and ethical use in mind is possible and necessary in safety and mission-critical domains like aerospace. Safe, trusted, and ethical use of AI are often used interchangeably; however, a system can be safely used but not trusted or ethical, have a trusted use that is not safe or ethical, and have an ethical use that is not safe or trusted. This manuscript serves as a primer to illuminate the nuanced differences between these concepts, with a specific focus on applications of Human-AI teaming in aerospace system control, where humans may be in, on, or out-of-the-loop of decision-making.

==> Sections/Ethics.tex <==
\section{Ethics} \label{ethics}
In this section, we summarize the ethical viewpoints of philosophy, research/engineering, and law on the use of AI through published documentation and literature. We expand on the primary ethical challenges researchers and engineers face in development, deployment, and use in machine learning, and create recommendations for ethical deployment. 
%In this section, we hope to address the ethical viewpoints of philosophy, research/engineering, and law on the use of AI through published documentation and literature. In philosophy, we expose the theory that society, more specifically the users and the operators of a ML in a MUMT are the source of an AI's ethical behavior. We expand on the primary  ethical challenges researchers and engineers face in development, deployment, and use in Machine Learning, and create recommendations for ethical deployment. \textcolor{red}{In research and engineering, we [talk about]..... In law, we [talk about]... [thanks I knew I forgot something -b]} 

% \texttt{[draft notes - Introduction to ethics in ML, discuss the differing definitions. Philosophy covers righteousness, wrongness, and decision factors. Engineering/Research covers ethical usage and development. DoD covers application and situation - trying to cover their ass basically so they don't get dinged. Recommendations on how to solve this is probably warranted.] }


\subsection{ML Ethics in Philosophy}

Philosophy on the subject of ethics concerns the morality of decisions, of right and wrong, good and evil. For the last decade, philosophers have become concerned with the rise of AI; in particular, how to apply concepts of right and wrong to artificial intelligence. In general, philosophers tackling ethics can subscribe to one of the 3 frameworks \cite{ethicsHAIT}, shown in Table \ref{tab:ethicframeworks}.

\begin{table}[hbt!]
\caption{Types of Ethics in Philosophy \cite{ethicsHAIT}\label{tab:ethicframeworks}}
\centering
\begin{tabular}{p{0.15\linewidth} | p{0.6\linewidth}}
\hline
%& Transition& & \multicolumn{2}{c}{}\\\cline{2-2}
Ethical Framework& Description \\\hline
Deontology& Right and wrong are set by a predetermined set of rules, and to find whether something is moral or ethical you can put the situation through those moral rules.\\
Virtue Ethics& A person or groups character, in particular if they have good traits or characteristics, affect their morality and decisions. \\
Consequentialism& The way a person or group forms their ethical belief is due to feedback from society or others on if an action was right or wrong.\\
\hline
\end{tabular}
\end{table}

These philosophical considerations help build the foundation of trust, and so in this section we hope to expand on 3 references from literature and philosophy, and find ways to apply their positions.

\subsubsection{The Golem of Prague}

The first example of the ethical considerations of the use and development of robotics traces back to the Golem, a fictitious creature originating from Jewish mythology. The Golem is a mythological creature which is made of clay or mud that becomes animated through prayer. The Golem have been used as a mythical creature and tale for many years, but the most common retelling comes from the 16th century Jewish myth, "The Golem of Prague". In that tale, Judah Loew ben Bezalel, the chief rabbi of Prague, created a clay automata to protect Prague and its Jewish population \cite{Spinoza}. The automata was given a name, and a simple set of instructions to protect the city and its citizens. The Golem patrolled the streets of Prague for 10 years, but eventually it is deactivated for one of 3 major reasons.

 The most common ending is that the Golem fulfilled its purpose and was sealed away in the attic of the Prague synagogue to be called upon in the future \cite{praguegolemhawaii}. However, 2 other popular tales have more relevance in terms of AI and have been brought up in modern literature as a potential ethical question. In Spinoza \cite{Spinoza} the Golem had experienced a malfunction of some sort to its base programming, misinterpreting its base instructions to create havoc on the local population. The hubris of the rabbi in creating an autonomous system that can have differing opinions on its programming has resurfaced in many ethical discussions even to the modern world \cite{golem-umich}. In another case, the Golem began to be used in tasks that it was not created to do, such as menial labor, and then rampaged in retaliation\cite{praguegolemhawaii}. This leads to questions as to whether the Golem was good or evil, considering the Golem itself was not programmed with the capability to perceive good or evil \cite{praguegolemhawaii}. 

But ultimately, what leads to the deactivation of the Golem in all stories is the trust the rabbi gives in the Golem to perform its function. It should be noted in all cases that the Golem is deactivated only when others perceive the Golem to have deviated from its mission. When the Golem malfunctions or performs unexpectedly, it breaks the trust between it and the users, such as when it deviated from its objectives, or when the mission was completed and it was no longer needed. The trust between the user and the Golem changed leading to the Golem being sealed. This legend has been the concern of multiple theologians and philosophers since, and creates the foundation for trust dynamics and ethical usage of automata. 

% \textcolor{red}{Summary for conference paper (usually around 12 pages total), but we should keep the longer version too: In the 16th century Jewish myth, ``The Golem of Prague" the chief rabbi uses prayer to animate a clay automata to protect the city and it's Jewish population via a simple set of instructions \cite{Spinoza}. A variety of tales detail how the Golem malfunctioned, including intentionally or unintentionally misinterpreting its programming and creating havoc on the local population, retaliating against menial labor tasks by rampaging city.  }

\subsubsection{MIT's Moral Machine and the 21st century Trolley Problem}
The trolley problem is a well known moral psychology question which was first introduced in 1967. The problem consists of a runaway train or trolley-bus that is about to cross a junction. At that junction, the trolley operator can make the decision to move the trolley, intentionally hitting 1 pedestrian, or do nothing and have the trolley crash, causing significantly more deaths. Both options are unethical, but the decision to take one life versus not being involved, or letting others die while sacrificing the few, is the basic ethical principle of the debate. Today, the trolley problem has resurfaced due to the rise of autonomous agents operating in closer proximity to humans, especially in the wake of autonomous cars. While initially just a starter for ethics debates, modern scientists use data driven psychology in order to understand the trolley dilemma, specifically by polling large groups of people on the situation in order to break down morality by location, gender, income gap, ethnicity, and other factors \cite{michigantrolley}. 

MIT has modernized the trolley problem concept into the MIT Moral Machine. The MIT Moral Machine \cite{mitmoral} is a website which presents ethical dilemmas an autonomous car could face and asks users from across the globe how the autonomous car should respond. In each ethical dilemma, the autonomous vehicle would be presented with 2 choices in which either the passenger, crossing pedestrian, or sidewalk pedestrian, would be killed, and varied the kind of person the car would kill by gender, occupation, and whether or not they were jaywalking. With more than 40 million decisions that were polled, MIT was able to break down how the public would see a autonomous car incident by ethnicity, gender, religion, and affiliation. Their paper \cite{mitmoral} discovered that there were major differences in what decisions people would make depending on the context and based on their country of origin. In general, people were more likely to spare larger groups than smaller groups, and spare humans over pets, but past that the cultural and economic variations greatly affected the outcomes. In practice, the paper outlines that regional differences had to be accounted for in design and ethical considerations of future autonomous cars. 
\newline

\subsubsection{Asimov and the 3 Laws}
The most well known ethical boundary in Robotics and Automation was created by Issac Asimov in 1942, known as the 3 Laws of Robotics. Issac Asimov wrote a series of short stories from 1942-1988 in which he explores the ethical and moral challenges robots would face, compiling them later into 2 major books,  \textit{I, Robot} \cite{robot} and \textit{Foundations} \cite{foundation}. In his stories, Asimov proposes the following 3 laws be programmed as the foundational starting piece for robots to behave ethically \cite{foundation}, so that all ethical decisions robots must consider can be resolved without malfunctions and the robot can continue its objective.

\vspace{10pt} \begin{enumerate}
    \item A robot may not injure a human being or, through inaction, allow a human being to come to harm. 
    \item A robot must obey the orders given it by human beings except where such orders would conflict with the First Law. 
    \item A robot must protect its own existence as long as such protection does not conflict with the First or Second Law.
\end{enumerate} \vspace{10pt}

Any modifications of these rules leads to operators experiencing strange or irrational behavior from their robots. But the 3 laws are just as much of a societal expectation as they are a programmable rule. \textit{Lost Little Robots} \cite{robot} suggests that letting the public know that one of the laws was modified in any way would lead to public outcry. In that story, because the robot was programmed with a different ethical foundation it behaved differently to other robots of the same model which operators did not expect and had to work around. Many years later, in \textit{The Caves of Steel} \cite{robot}, the 3 laws have become ingrained into expectations for robot behavior and robots who modify that base programming are flagged as outcasts of society or serious hazards. Society and Robots carry the expectation of following these ethical boundaries.

It is that balance in ethical boundaries between societies and the robots that Asimov began to focus his writing around, and how inadequate they were as moral grounds. In \textit{Runaround} \cite{robot} the robot's strict adherence to the 2nd and 3rd laws led to the robot being stuck in a dilemma that led to a human in danger. Asimov later explores society manipulating the interpretation of the 3 laws in Foundations. The \textit{Naked Sun} \cite{robot}\cite{foundation} introduces a human faction called the Solarians, who are politically distinct from other humans, manipulated the 1st law by not informing ship algorithms that human lives are placed in danger due to their actions. Later, in \textit{Foundations and Earth} \cite{foundation}, Solarian robots are programmed with a definition of human as only empire citizens, shunning outsiders from the planet. This is important because the first person to break Asimov's rules of robotics is Asimov, who argues the definition of ethics changes in robots as society interprets it.


\subsubsection{ML Ethics in Philosophy Summary}
What the Golem, the MIT Moral Machine, and Asimov's writings demonstrate, is an approach of modern philosophy. What an individual considers is a rational or ethical decision can be up for interpretation, but as a whole societies and organizations share differences in what they define as moral and their ethical boundaries. In the MIT Moral Machine \cite{mitmoral}, countries with stronger rules of law were less likely to spare pedestrians, countries with lower economic output were less likely to spare people based on their profession, and other similar factors. People in places where society places different values on emotion \cite{michigantrolley} also plays a factor when facing an ethical dilemma. As Asimov explores, societies, even when they follow the same ethical guidelines, will have different interpretations \cite{foundation} of ethics and use those interpretations in unforeseen methods\cite{robot}.

In conclusion, the users of an algorithm, whether it be an individual, group, department or society, lays their own expectations of how robots will behave and if they behave ethically. Therefore, any algorithm attempting to resolve ethical dilemmas is evaluated by it's users, and therefore should share the ethical boundaries of its users demographics. This statement can be considered controversial in cases where algorithms are applied outside of their country of origin, but the alternative is a lack of trust between the user and the algorithm in terms of ethical boundaries, something of which must be addressed early. If practical, users should be polled during the development of algorithms to factor in their ethical considerations before wide scale deployment.

\subsection{ML Ethics in Research and Engineering}
While philosophy considers the ethical and moral boundaries of AI, ethics in Research and Engineering care more about if the usage of a particular platform was ethical, or if their system was applied ethically in a situation. Most engineering literature define ethics as set rules of right and wrong, following the philosophical principle of Deontology \cite{asmeethics}. Researchers and Engineers are concerned more with developing systems to behave ethically, to make sure their systems are deployed ethically, and make sure their research does not violate ethical considerations. In this subsection we address ethical design and usage of AI, and how those ethical boundaries are currently being challenged. 

\subsubsection{Ethical Behavior in ML}

One of the currently expanding fields of research in ML is designing ethical behavior into algorithms during development and deployment. The debate of what is defined as ethical among engineers and users can have real consequences, leading to resignations, layoffs, and firings of talented individuals who carry concerns that their organization is not operating ethically, or leading to fear of adoption from organizations. The primary focus as of publishing has been on 3 subjects: 1) whether algorithms can be programmed with ethical behavior, 2) dealing with bias in algorithm data, and 3) how organizational ethics, particularly around privacy, affect the Manned-AI Team decisions.  

There is a substantial amount of literature in ML focused on ensuring that ML behaves and acts in ways considered ethical. The major papers focuses around a debate questioning if AI can even be programmed to act ethically or not. On one hand, \textit{Ethics in Human-AI Teaming} \cite{ethicsHAIT} suggests that ML algorithms can and should be programmed with a ethics decision algorithm. However, others argue that since ethics is still a ongoing debate in philosophy, it's not really possible to code those principles to ML \cite{forbesethics}. David M. Tate of the Institute for Defense Analysis \cite{idapaper} also postulates that ethics is more about trust and transparency. In all cases, it matters more that there is trust between the human and the ML to not violate the human's ethical boundaries\cite{trustoperationalcontext}, which will be expanded in further detail in Section \ref{sec:Trust}. 

Another important problem in ethical design of ML models is removing bias from algorithms. Bias in ML has become a critical point of contention at Alphabet Inc. (parent company of Google,NASDAQ: GOOGL) \cite{googlefiringethicist} as well as other companies and even government agencies. The National Institute for Standards and Technology (NIST) has put together a publication focuses on identifying and managing bias in AI \cite{nistbias} which can be broken down into 3 types found in Table \ref{tab:table2}. These biases influence each other in ways that lead to real world consequences.

\begin{figure}[hbt!]
\caption{\label{tab:table2}: Types of Bias in AI \cite{nistbias}}
\centering
\begin{tabular}{p{0.15\linewidth} | p{0.6\linewidth}}
\hline
%& Transition& & \multicolumn{2}{c}{}\\\cline{2-2}
Type of Bias& Description \\\hline
Systemic Bias& Systemic bias comes from information sourced from history, society, or institutions. This mostly manifests in the data that arrives from these sources and the bias this data was collected with. \\
Human Bias& Human Bias comes from the user and the biases the user has towards their interaction, as the bias of the user or organization will manifest in the AI algorithm.\\
Statistical Bias& Statistical Bias comes from the development of the AI, particularly in the use of the system, the sampling and filtering of the algorithm, and the AI model selection.\\
\hline
\end{tabular}
\end{figure}

In one example \cite{ricespeechethics}, training data that was skewed in credit card history unfortunately led to biases against women in applying for Apple/Goldman Sach's credit card line. However, the training data did not carry gender as an input, leading to confusion as to how bias was introduced. In another case \cite{neartermAIethicalmatrix}, software used to evaluate risk for parole release rated people based on race due to bias from the input data. Both cases showed that training data and biases hidden in the training data became modified and amplified through the ML model \cite{nistbias}, leading to ethical problems later on. In The \textit{Near-Term Artificial Intelligence and the Ethical Matrix} \cite{neartermAIethicalmatrix} proposes engineers use the feedback from data generated by stakeholders on the bias of the system, and use that to create a chart outlining the chance of false positives and false negatives \cite{neartermAIethicalmatrix}. This ethical matrix provides transparency to operators and users, allowing for developers to have a goal to work towards in reducing bias in the system.  Alphabet, INC and OpenAI use a similar system called PALMS which retrains the ML to remove unsafe behavior, expanded more upon in \ref{sec:LaMDASafety}.However, \textit{AI and Ethics} \cite{ethicsHAIT} postulates that it's not just enough for ML to be adjusted afterwards, and proposes an ethical safety system must be built in during the design phase. The paper calls this system the Agent, Deed, Consequence (ADC) model, and it combines 3 philosophical models to formulate a decision on if an action is ethical or not \cite{ethicsHAIT} in Figure \ref{chart:ADCModel}.

\begin{figure} [hbt!]
\centering
\includegraphics[width=.5\textwidth]{Figures/Modified AEIT Diagram.png}
\caption{\label{chart:ADCModel}Flow chart of modified of Agent, Deed, Consequence model}
\end{figure}

%[a section on the ethics of the basically enslavement of sentient AI would go here if it was covered by anyone, but there is almost zero worthwhile academic literature on this subject]

\subsubsection{Responsible Use of ML}
Most of the international debate over AI is focused on whether the usage of ML is ethical, rather than checking if an AI behaves ethically. As ML and AI become more prolific, the debate over using AI in specific applications has become increasingly contentious. We can use this opportunity to look at some relevant examples, how users or observers saw this use as unethical, and how to account for that in future deployment and usage of ML algorithms. 

The most recent debate as of 2022 has been over the development and deployment of \textit{neural network chatbots}, some of which use RL to try and predict the next sentence in a conversation with another human \cite{googlelamda}. In 2014, a computer model was the first to pass the Turing test, a test where a series of interrogators vote anonymously on if a program is human or not \cite{guardianturing1}. Even though the program passed the test while being relatively simple and by pretending to be a sassy 13 year old child \cite{guardianturing2}, the fact that more than 30 percent of questioners believed the bot to be real raised ethical concerns at the time. More recently, large language models, neural networks trained using data from a specific language, have caused controversy at Alphabet due to an engineer claiming their model, LaMDA, is sentient \cite{lamdainterview}. Alphabet also raised concerns about LaMDA in it's development phases and began to implement safety measures in training LaMDA to not produce unethical behavior \cite{googlelamda}. In the safety section of their paper \cite{googlelamda}, they outlined how their safety system and criteria for LaMDA works. We expand more upon how that safety system works in \ref{LaMDASafety}.

It becomes part of ethical use of machine learning to make sure input data is sanitized and safety measures are built into data collection tools to prevent it's unethical use. Without these safety mechanisms AI will received biased or unsafe data to train on and behave unethically, such as the problem with Microsoft Tay\cite{microsofttay}, an experiment where a ML algorithm was allowed to interact with the public through Twitter, with little safety filters built in. With coordinated efforts by twitter users, Tay received poisoned data and displayed racist and misogynistic tweets, attacking a game developer \cite{microsofttay}.  Another unfortunate use case of chatbots was created by AI researcher Yannic Kilcher, created a GPT-J learning model he called "GPT-4Chan", which trained off of user data generated on the infamously toxic forum 4chan \cite{4chanai} and then allowed the algorithm to post to the same forum. This raised multiple ethical concerns as not only was the bot posting inappropriate responses \cite{4chanai} but the system was released in real time against other users and also open sourced, allowing others to download and use the unethical AI in locations it was not trained for. This led to OpenAI's GPT-3 being redeveloped to filter out unethical behavior\cite{4chanai}, in which Alphabet's LaMDA adopted the same model \cite{googlelamda}. 

Another concern over the ethical usage of ML in interacting with humans is over the use of \textit{facial recognition}. Concern over facial recognition fits into 2 categories: 1) concern over bias and 2) concerns in widespread deployment. In 2017, 2 MIT researchers put together a report called \textit{Gender Shades} \cite{gendershades}, which highlights that facial recognition and detection were biased against minorities of darker skin color. The paper tested multiple facial recognition algorithms being developed by Microsoft, IBM, and others which were being used in government applications leading to a temporary halt and audit of their use \cite{gendershades}. This has manifested into concerns in widespread deployment of facial recognition, highlighted to the public by the HBO series Last Week Tonight \cite{johnoliverrant}. Because operators were more likely to trust the ML algorithm than the subjects the algorithm was being used on, a lack of feedback over errors resulted in multiple false positives going unnoticed.

The last major concern over ethical use has been in the deployment and ethics of robots in combat and defense roles, primarily focused on whether robots should be allowed to harm others, and what the privacy concerns are over mass surveillance using ML and robot platforms. Axon Enterprise, Inc, caused major controversy when they announced the development of a flying taser, leading to a majority resignation of their ethics board \cite{axonresignation}. The project was considered unethical use of autonomous platforms, as the goal of the project was to have autonomously followed, targeted, and tasered a perpetrator without human input. They intended \cite{axonresignation} to deploy these robots around schools and government facilities with camera platforms to track people carrying firearms in illicit places. This lack of human input over autonomous platforms raised many red flags, especially in civilian use, leading not just engineers within the project but multiple operators of axon products to raise objections \cite{lit}, lower societal and operator trust over robotics in general. The product would have been seen as too politically and ethically radical. The Red Cross has also raised recommendations that autonomous platforms must have a human operator make the final decision to take action which influences another life, and operate with a human in the loop \cite{icrcautonweapons}.

\subsection{ML Ethics in Application}
As ML proliferates, multiple government and even international organizations have begun releasing guidelines on ethical AI usage and development. These organizations are setting the standard both at home and abroad for their organizations, which affects their algorithms ethical framework and use. This subsection outlines the responsibility of agents in the field and how organizations define ethical usage of AI.

\subsubsection{International Law}
The International Committee of the Red Cross have taken the opinion that autonomous platforms follow the Martens Clause of the 1907 Hague Convention \cite{icrcautonweapons}. The Martens Clause is a catch all clause which says that, barring any direct regulation, civilians and combatants follow rules derived from established customs, human principles, and public conscience. It has been interpreted in this context to overlap that the ethical and legal rules of an autonomous weapon is that of the operator country \cite{icrcautonweapons}. If an autonomous agent was no longer in command or control by the operator country, the robot would be subject to regulations of the operator country and the operator would take the blame for any unethical actions the agent carried out. This opinion has not been codified in any other international law body, notably the United Nations Security Council and International Court of Justice, and will likely be a point of contention only when a situation develops. 

\subsubsection{US Government Principles}
The United States Government and it's various departments have begun putting together rough outlines for the ethical and responsible use of AI. Initially, the Department of Defense's Innovation Board released a series of 5 guidelines of ethical principles that were officially adopted in 2020 by the former Secretary of Defense\cite{dodethicalprinciples}. A year later, two industry consultants - Gartner Inc and the American Council for Technology Industry Advisory Council (ACT-IAC), developed very similar ethical principles. All principles are summarized in Table \ref{tab:govethics}.

\begin{table}[hbt!]
\caption{\label{tab:govethics} Compiled ethical principles related to AI \cite{nasaaiethics}}
\centering
\begin{tabular}{p{0.34\linewidth} | p{0.3\linewidth}| p{0.3\linewidth}}
Department of Defense Innovation Board& Gartner Consulting, Inc.& ACT-Industry Advisory Council\\\hline
Responsible& Secure and Safe& Bias\\
Equitable& Fair& Fair\\
Traceable& Explainable and Transparent& Transparent\\
Governable& Accountable& Responsible\\
Reliable& Human-Centric, Societally Beneficial& Interpretable\\
\hline
\end{tabular}
\end{table}


    \textcolor{red}{YO INSERT THIS}
https://www.researchgate.net/publication/318671145_Society-in-the-Loop_Programming_the_Algorithmic_Social_Contract


NASA expanded on the Gartner Consulting principles and merged the DoD and the ACT-IAC principles into 6 overall recommendations that outline most of the government policies\cite{nasaaiethics}, defined as follows:

\begin{itemize}
    \item Fair: AI must mitigate discrimination, manipulation, and bias.
    \item Explainable and Transparent: AI must make decisions that are considered rational and understandable.
    \item Accountable: Humans must be able to provide oversight on algorithms.
    \item Secure and Safe: Respect privacy and do no harm.
    \item Human-Centric: Must follow current laws and be beneficial.
    \item Scientifically and Technically Robust:  Must undergo rigorous testing that is well documented.
\end{itemize}

%table version of itemized list
%\begin{table}[hbt!]
%\caption{\label{tab:NASAEthics}: NASA Framework for Ethical Use of AI \cite{nasaaiethics}}
%\centering
%\begin{tabular}{p{0.28\linewidth} | p{0.5\linewidth}}
%\hline
%& Transition& & \multicolumn{2}{c}{}\\\cline{2-2}
%Fair& AI must mitigate discrimination, manipulation, and bias. \\
%Explainable and Transparent& AI must make decisions that are considered rational and understandable.\\
%Accountable& Humans must be able to provide oversight on algorithms.\\
%Secure and Safe& Respect privacy and do no harm.\\
%Human-Centric& Must follow current laws and be beneficial.\\
%Scientifically and Technically Robust& Must undergo rigorous testing that is well documented.\\
%\hline
%\end{tabular}
%\end{table}

% \subsubsection{ACT3 Opinion}
% [this section may not be releasible?]

% https://arxiv.org/ftp/arxiv/papers/2103/2103.12638.pdf 
% [discussions in Quest]
% [discussions in mattermost]
% [discussions with terry]

\subsection{Recommendations for Ethical design}

From aspects of philosophy and literature, as well as from use cases and examples of ethical and unethical behavior compiled in this section, we can build upon the principle that society, in particular the beliefs and ethics users in a society follow, affect the trust between algorithms and humans. Any system will have to account for the fact that those ethical boundaries change with time, location, and operator. 

\vspace{10pt} \begin{enumerate}
    \item The algorithm and the operator agree on a similar set of ethical values and boundaries with both aware of those values.
    \item That the algorithm and operator build trust that the user or the algorithm will not violate agreed upon ethical boundaries or demonstrate bias against certain users.
    \item The operator has a feedback mechanism with the developer and/or with the algorithm to discuss and prevent ethical violations.
    \item The operator needs to be given information or training on the consequences of improper use of the algorithm. 
\end{enumerate} \vspace{10pt}

These recommendations can be implemented through multiple different methods such as through polling users during development, creating or following an ethical guideline, and adopting safety and control mechanisms into the ML algorithm that prevent bad or inappropriate data from being inputted. But the most important method for the ML algorithm to operate ethically is trust between the user and the ML, which requires a clear set of communications between both parts of a Human-AI team. 


==> Sections/Safety.tex <==
\section{Safety}
\textcolor{red}{An introduction paragraph will go here. Not sure what yet, please ignore.}

\subsection{Importance of Safety in Automation}
In order to understand the current climate in automation, it's best to look at primary examples of safety in manned-unmanned teaming from a wide variety of industries. 

\subsubsection{Uber Self-Driving SUV}
In March of 2018, a Self Driving Car commissioned by Uber and manufactured by Aurora Innovation hit a pedestrian holding a bicycle in the dead of night, marking the first ever death of a human from an autonomous vehicle \cite{ubercrashntsb}. The National Transportation and Safety Bureau (NTSB) conducted a report which found that while the driver and pedestrian were both at fault, design faults in how Aurora Innovation implemented their autonomous driving system lead to the safety problems that caused the incident. This sets the precedence for

%https://money.cnn.com/2018/03/19/technology/uber-autonomous-car-fatal-crash/index.html?iid=EL
%https://web.archive.org/web/20190831200841/https://www.ntsb.gov/investigations/AccidentReports/Reports/HWY18MH010-prelim.pdf Originally %https://www.ntsb.gov/investigations/AccidentReports/Reports/HWY18MH010-prelim.pdf 
%https://en.wikipedia.org/wiki/Death_of_Elaine_Herzberg 
%[I was the operator - WIRED interview and Op-Ed] https://www.wired.com/story/uber-self-driving-car-fatal-crash/
%[NTSB investigation uber crash https://www.ntsb.gov/investigations/accidentreports/reports/har1903.pdf ]

\subsubsection{Auto GCAS}
The Automatic Ground Collision Avoidance System, better known as Auto GCAS, is an example of where MUMT works effectively. Auto GCAS is a system designed for the F-16 that attempts to level the aircraft when the aircraft is following a trajectory that will collide with the ground. 


%https://www.popsci.com/story/technology/agcas-technology-saves-pilots-lives/ 
%https://www.lockheedmartin.com/en-us/products/autogcas.html
\subsubsection{Boeing 737-800 MCAS}

%https://www.youtube.com/watch?v=wXMO0bhPhCw 

\subsubsection{Chemical Safety Board Incidents}


\subsubsection{Google's LaMDA safety system and the Microsoft Tay incident} \label{sec:LaMDASafety}

An increasing relevant section of safety in autonomous systems is in managing safe responses of large language models and chatbots. Google has been working to implement a strong safety system in their LLM, LaMDA \cite{googlelamda}. Previous chatbots that were trained on internet messages were prone to making immoral or inflammatory remarks, as in the case with Microsoft Tay \cite{microsofttay}. Microsoft Tay is a case study in it's own that has been outlined in \ref{ethics}, but in summary without any filtration system or human feedback system built into Microsoft's Tay chatbot, it began to output incredibly inappropriate remarks. Google took the time to develop what they defined as safety, primarily focusing on preventing risks of harm and avoiding unjust impacts on groups of people. They used a safety management system called PALMS, created by OpenAI, to then filter out bad behavior \cite{palmssafety}. PALMS feeds user expectations of a chatbots response back into the starter event and tuning system, removing answers that may be considered dangerous or unethical. With it, they were able to prevent LaMDA from being released with inappropriate behavior \cite{palmssafety} \cite{googlelamda}.

\subsection{Noticing Safety Problems}

\subsubsection{}

\subsubsection{Instructional Requirements}
Boeing’s **** up

\subsubsection{Noticing Errors}
One of the major problems with designing safety systems is clear communication and alarm systems, primarily in applications where automation is mandatory. On March 28th, 1979, at 4:00AM, the Three Mile Island nuclear reactor began a series of events which led to America's worst nuclear meltdown. 7 months later, the US Presidential Commission on the Accident at 3 Mile Island released their report. Of the 3 major factors that caused the meltdown, one of the problems was a design fault not of the reactor, but of the operator console \cite{tmireport}. 

%Three Mile Island Report

%Swarm Paper and Other paper


%https://www.hsdl.org/?abstract&did=769775 
In the Pryor Trust/Gas well, the alarm system managing the blowout preventer was disabled for 14 hours before the fracking well exploded.
%://www.csb.gov/pryor-trust-fatal-gas-well-blowout-and-fire/ 
\subsubsection{Communicating Trust}

Operators need to have a path to speak to the developers about problems that operators know will be looked at and trust patches for will come. 

\subsection{Building in Safety}
While there are discussions as to whether trust\cite{idapaper}  and ethics\cite{ethicsHAIT} can be built into a system, safety is agreed upon by almost all research to be a necessary design criteria of any autonomous system interfacing in real-world scenarios. 

\subsubsection{Aerospace Hazard Analysis Tools}
Traditional aerospace analysis tools have been 

\subsubsection{STAMP Analysis}

\subsubsection{Run-Time Assurance}

\subsubsection{PALMS System}

\subsubsection{Human-AI Safety Criteria}
A critical section of designing safety with autonomous systems that cannot be ignored is the interaction of the algorithm with the human. The NTSB Highway Accident report\cite{ubercrashntsb} outlined problems with safety between the human and an autonomous vehicles, the major problem being automation complacency. Automation complacency comes from a Parasuraman paper \cite{paracomplacencybias}, which Lee and See categorizes appropriate reliance \cite{leeandsee}. Appropriate reliance is related to trust, when a user overtrusts or undertrusts ML they can stop monitoring the ML appropriately, which can cause failure. The NTSB noticed that autonomous vehicles, particuarly in the uber case, 


\begin{figure} [hbt!]
\centering
\includegraphics[width=.8\textwidth]{Figures/PALMS system steps.png}
\caption{\label{chart:PALMS}Overview of OpenAI's PALMS safety system with modified phase titles \cite{palmssafety}}
\end{figure}

\subsection{Lessons and Recommendations}
Learning from all, one of the critical factors in safety and trust in implementing any algorithm that has the ability to influence the inputs of a vehicle and/or take control of a vehicle is to ma (not a sentence rip) 

The following recommendations are compiled from readings and should be taken as the foundation for how AIs should operate in future AI development to build trust between a user and it’s AI algorithm. 
\vspace{10pt} \begin{enumerate}
\item The operators shall be informed on the functionality and limitations of any algorithm that has the ability to influence operator input. 
\item The algorithm shall communicate with operators prior to and while influencing the system controls. 
    \begin{itemize}
        \item The algorithm should have an output to the user that the user can monitor and understand.
        \item The algorithm should provide auditory and/or visual notices when the algorithm influences the system.
        \item Example Auto GCAS
    \end{itemize}

\item The algorithm shall be transparent to the operator on when the algorithm wants to influence a system and its reasoning for influencing the system.
    \begin{itemize}
        \item For example in Auto GCAS, chevrons appear on the heads up display to indicate that the Auto GCAS is about to activate a recovery maneuver.
    \end{itemize}
  
\item The human operator shall be able to control and influence the operation of all algorithms which have the ability to influence the system. 
\item The user and the algorithm can recognize when it is about to violate critical boundaries in minimum and maximum viable operations. 
    \begin{itemize}
        \item Example  -  MCAS
    \end{itemize}
\item The operators shall constantly monitor algorithms when the algorithm is directing the system.
    \begin{itemize}
        \item This can be met by the algorithm monitoring the user and requiring the user to be physically engaged.
        \item This could be a requirement that the system validates that the operator is monitoring the algorithm. For example, Tesla requires hands on the wheel through the use of a pressure sensor.
        \item This can also be where the algorithm is observing the user for fatigue, such as through the use of heart rate monitors, eye tracking, or similar systems.
        \item In some cases, this is met by training the operator. 
    \end{itemize}
\end{enumerate} \vspace{10pt}


\section{Safety}
One of the key challenges in developing autonomous systems, especially neural network control systems (NNCS), producing evidence that the system will be safe. While there are some advances in reachability for neural networks, the results are very limited, and the current state of the art is not capable of completely verifying safety of autonomous systems.


This section investigates challenges in safety for manned-unmanned teaming (MUMT).



% \begin{center} \textbf{Work on this section is being postponed so that other sections can be completed first. What can be found below is the headers and rough outline of the section.} \end{center}
\subsection{Examples of Safety for Automatic and Autonomous Systems}


\subsubsection{Uber Self-Driving SUV}
%In March of 2018, a Self Driving Car commissioned by Uber and manufactured by Aurora Innovation hit a pedestrian holding a bicycle in the dead of night, marking the first ever death of a human from an autonomous vehicle \cite{ubercrashntsb}. 

In March of 2018, a Self Driving Car commissioned by Uber and manufactured by Aurora Innovation hit a pedestrian holding a bicycle in the dead of night, marking the first ever death of a human from an autonomous vehicle \cite{ubercrashntsb}. The National Transportation and Safety Bureau (NTSB) conducted a report which found that while the driver and pedestrian were both at fault, design faults in how Aurora Innovation implemented their autonomous driving system lead to the safety problems that caused the incident.

%Based on the recommendations of the NTSB,
%https://money.cnn.com/2018/03/19/technology/uber-autonomous-car-fatal-crash/index.html?iid=EL
%https://web.archive.org/web/20190831200841/https://www.ntsb.gov/investigations/AccidentReports/Reports/HWY18MH010-prelim.pdf Originally %https://www.ntsb.gov/investigations/AccidentReports/Reports/HWY18MH010-prelim.pdf 
%https://en.wikipedia.org/wiki/Death_of_Elaine_Herzberg 
%[I was the operator - WIRED interview and Op-Ed] https://www.wired.com/story/uber-self-driving-car-fatal-crash/
%[NTSB investigation uber crash https://www.ntsb.gov/investigations/accidentreports/reports/har1903.pdf ]

\subsubsection{Auto GCAS}
The Automatic Ground Collision Avoidance System (Auto GCAS) is an example of where MUMT works effectively. Auto GCAS is a system designed for the F-16 that attempts to level the aircraft when the aircraft is following a trajectory that will collide with the ground. 

%https://www.popsci.com/story/technology/agcas-technology-saves-pilots-lives/ 
%https://www.lockheedmartin.com/en-us/products/autogcas.html
\subsubsection{Boeing 737-800 MCAS}

%https://www.youtube.com/watch?v=wXMO0bhPhCw 

\subsubsection{Chemical Safety Board Incidents}

\subsubsection{Google's LaMDA safety system and other Chatbots} \label{sec:LaMDASafety}

Chatbots and their interactions with humans has also been up 

An increasing relevant section of safety in autonomous systems is in managing safe responses of large language models and chatbots. Google has been working to implement a strong safety system in their LLM, LaMDA \cite{googlelamda}. Previous chatbots that were trained on internet messages were prone to making immoral or inflammatory remarks, as in the case with Microsoft Tay \cite{microsofttay}. Microsoft Tay is a case study in it's own that has been outlined in \ref{ethics}, but in summary without any filtration system or human feedback system built into Microsoft's Tay chatbot, it began to output incredibly inappropriate remarks. Google took the time to develop what they defined as safety, primarily focusing on preventing risks of harm and avoiding unjust impacts on groups of people. They used a safety management system called PALMS, created by OpenAI, to then filter out bad behavior \cite{palmssafety}. PALMS feeds user expectations of a chatbots response back into the starter event and tuning system, removing answers that may be considered dangerous or unethical. With it, they were able to prevent LaMDA from being released with inappropriate behavior \cite{palmssafety} \cite{googlelamda}.

\%subsection{Noticing Safety Problems}

%\subsubsection{}

%\subsubsection{Instructional Requirements}
%Boeing’s **** up
\subsubsection{Three Mile Island}
One of the major problems with designing safety systems is clear communication and alarm systems, primarily in applications where automation is mandatory. On March 28th, 1979, at 4:00AM, the Three Mile Island nuclear reactor began a series of events which led to America's worst nuclear meltdown. Seven months later, the US Presidential Commission on the Accident at 3 Mile Island released their report. Of the 3 major factors that caused the meltdown, one of the problems was a design fault not of the reactor, but of the operator console \cite{tmireport}. 
%
%Three Mile Island Report
%
%Swarm Paper and Other paper
%
%
%https://www.hsdl.org/?abstract&did=769775 
In the Pryor Trust/Gas well, the alarm system managing the blowout preventer was disabled for 14 hours before the fracking well exploded.
%://www.csb.gov/pryor-trust-fatal-gas-well-blowout-and-fire/ 
%\subsubsection{Communicating Trust}

%Operators need to have a path to speak to the developers about problems that operators know will be looked at and trust patches for will come. 


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Building Safety}

Safety can be divided into two different kinds of constraints: soft safety constraints and hard safety constraints. Soft safety constraints are desirable conditions for the system, but are not strictly enforced, for example, at least one of the aircraft in a two ship formation should have line of sight to the other aircraft. Hard safety constraints should never be violated, such as that the wingman aircraft shall always maintains safe separation with a lead aircraft. Soft safety can be added by training the autonomous agents to be safe; however this does not guarantee safety. An alternative approach of particular merit for hard safety constraints is to monitor the autonomous system behavior at runtime and intervene when necessary to assure safety, an approach known as run time assurance.

\subsubsection{Engineering Hazard Analysis Tools}

\subsubsection{STAMP Analysis}

\subsubsection{Run-Time Assurance}

\subsection{Lessons and Recommendations}
%Learning from all, one of the critical factors in safety and trust in implementing any algorithm that has the ability to influence the inputs of a vehicle and/or take control of a vehicle is to ma (not a sentence rip) 

The following recommendations are compiled from readings.% and should be taken as the foundation for how AIs should operate in future AI development to build trust between a user and it’s AI algorithm. 
\vspace{10pt} \begin{enumerate}
\item The operators shall be informed on the functionality and limitations of any algorithm that has the ability to influence operator input, or decisions or behavior of the autonomous system. 
%\item The algorithm shall communicate with operators prior to and while influencing the system controls. 
%\begin{itemize}
%  \item The algorithm should have an output to the user that the user can monitor and understand.
%  \item The algorithm should provide auditory and/or visual notices when the algorithm influences the system. 
%\end{itemize}

%\begin{itemize}
%  \item For example, previous ground collision advisory systems used auditory warnings such as "pull up" or "altitude." Auto GCAS uses a number of visual cues to keep the pilot informed of it's state, the most important of which is arguably a set of chevrons that come in from the sides and meet in the middle when the system activiates. 
%\end{itemize}

\item The algorithm shall be transparent to the operator on when the algorithm wants to influence a system and its reasoning for influencing the system.
\begin{itemize}
  \item For example in Auto GCAS, chevrons appear on the heads up display to indicate that the Auto GCAS is about to activate a recovery maneuver.
\end{itemize}
 
\item The human operator shall be able to control and influence the operation of all algorithms which have the ability to influence the system. 
%\item The user and the algorithm can recognize when it is about to violate critical boundaries in minimum and maxiable viable operations. 
 % \begin{itemize}
  %\item Example - MCAS
  %\end{itemize}
%\item The operators shall constantly monitor algorithms when the algorithm is directing the system.
%  \begin{itemize}
%  \item This can be met by the algorithm monitoring the user and requiring the user to be physically engaged. 
%  \item This could be a requirement that the system validates that the operator is monitoring the algorithm. For example, Tesla requires hands on the wheel through the use of a pressure sensor.
%  \item This can also be where the algorithm is observing the user for fatigue, such as through the use of heart rate monitors, eye tracking, or similar systems.
%  \item In some cases, this is met by training the operator. 
%  \end{itemize}
\end{enumerate} \vspace{10pt}

==> Sections/Trust.tex <==
\section{Trust} \label{sec:Trust}

In this section we hope to explore the literature concerning trust in manned-unmanned teams, how that trust is built experimentally, and the challenges in trusting any complex system. 
% \begin{center} \textbf{Work on this section is being postponed so that other sections can be completed first. What can be found below is the headers and rough outline of the section.} \end{center}

\subsection{What is Trust?}

\subsubsection{Competing Definitions}

%\textcolor{red}{INSERT THIS!!!} https://www.federalregister.gov/documents/2020/12/08/2020-27065/promoting-the-use-of-trustworthy-artificial-intelligence-in-the-federal-government

%Trust as Vulnerability vs Trust as Expectations (Reliability)


%\subsubsection{Overview of Trust Dynamics}

%\begin{figure} [hbt!]
%\centering
%\includegraphics[width=0.9\textwidth]{Figures/Trust Diagram.png}
%\caption{Flow Chart of Trust building, divided into 4 major phases and compiled from multiple articles.}
%\end{figure}



\subsection{The Beginnings of Trust}
% [Parasuraman papers] [trust of military system in automated context]

\subsubsection{Knowledge Level}


\subsubsection{Automation Bias}


\subsubsection{Human-AI Interface}

\cite{airbusrefuel}

Alongside traditional machine interface design we've begun to see a unique trend where humans anthropomorphize robots and their unique characteristics.  While science fiction has been concerned with this since the 1950s \cite{robot}, in the early 2000s we began to see real world cases of humans expressing positive traits onto robots based on their features and behavior. The first documented case of this is with iRobot's Roomba platform, a robot vacuum which user gave positive traits and characteristics due to it's function and proximity to users \cite{roomba}. Not only did users want to personalize their unique roomba, operators assigned Roombas specific names and considered them similar to house pets, and became more willing to tolerate more extraneous behavior even compared to other cleaning robots \cite{roomba} due to their nonthreatening nature and positive contribution to the household. The Army Research Laboratory has expanded this concept further, finding similarities in Human-AI Teaming and Human-Animal Trust \cite{humananimal}. If the robot interacted with humans in a friendly way on occasion, if the errors it made were not severe, if the operator underwent training with the robot, if it was `cute' in either behavior or design, and if the environment the human and robot operated in was non-threatening, operators were more likely to accept unpredictable behavior. This does lead to an avenue for future research for using avatars or in-person analogs to symbolize AI, which IBM has begun researching with Watson \cite{ibmwatson}. However, it should probably not be explored without having an engineering review on the exact application where the HAIT would need to have the ML algorithm be equipped with a virtual or physical avatar. There are going to be ethics questions if a ML is equipped with an avatar that does not work with the environment or situation the ML is deployed in.


\subsection{Predictability, Reliability and Trustworthiness}
% Lee and See 
%Rosseau

\subsection{Foundational Trust}
%IDA paper
%Ethics Paper 

\subsubsection{User Workload}

\subsubsection{Safety Aspects}

\subsubsection{Blame and Legal Ramifications}
%[I was the operator - WIRED interview and Op-Ed]
\subsection{Usage}
We should probably outline this section as the "Parasuraman papers" since this is basically all his. 
http://web.mit.edu/16.459/www/parasuraman.pdf 

\subsubsection{Overtrust}
%[I was the operator - WIRED interview and Op-Ed]
\cite{ubercrashntsb}
%https://www.researchgate.net/publication/47792928_Complacency_and_Bias_in_Human_Use_of_Automation_An_Attentional_Integration 

\subsubsection{Loosing Trust and Undertrust}

\subsection{Recommendations for Trust Dynamics}

\subsubsection{Human-AI Feedback}
Countinous Feedback from users on
\subsubsection{Autonomous Readiness Level}

\subsubsection{Trust Exercises?}

